Can Program Synthesis be Used to Learn Merge Conflict Resolutions? An Empirical Analysis

Forking structure is widespread in the open-source repositories and that causes a significant number of merge conflicts. In this paper, we study the problem of textual merge conflicts from the perspective of Microsoft Edge, a large, highly collaborative fork off the main Chromium branch with significant merge conflicts. Broadly, this study is divided into two sections. First, we empirically evaluate textual merge conflicts in Microsoft Edge and classify them based on the type of files, location of conflicts in a file, and the size of conflicts. We found that ~28% of the merge conflicts are 1-2 line changes, and many resolutions have frequent patterns. Second, driven by these findings, we explore Program Synthesis (for the first time) to learn patterns and resolve structural merge conflicts. We propose a novel domain-specific language (DSL) that captures many of the repetitive merge conflict resolution patterns and learn resolution strategies as programs in this DSL from example resolutions. We found that the learned strategies can resolve 11.4% of the conflicts (~41% of 1-2 line changes) that arise in the C++ files with 93.2% accuracy.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> code.tex <==
%DownstreamSpecificTest: {let dup = FindMatch(x, [""]) in Apply(Check(dup, [0, 5, 6]), Concat(Remove(SelectUpstream(x), SelectDup(dup, 0)), Remove(SelectDownstream(x), SelectUpstream(x))))}
% Duplicate in downstream: {let dup = FindMatch(x, [""]) in Apply(Check(dup, [2]), Concat(Remove(SelectUpstream(x), SelectDownstream(x)), Remove(SelectDownstream(x), SelectDup(dup, 2))))}

% Duplicate in downstream: {let dup = FindMatch(x, [""]) in Apply(Check(dup, [2]), Concat(Remove(SelectDownstream(x), SelectDup(dup, 2)), Remove(SelectUpstream(x), SelectDownstream(x))))}

% Duplicate in downstream and upstream: {let dup = FindMatch(x, [""]) in Apply(Check(dup, [0, 5]), Concat(Remove(SelectUpstream(x), SelectDup(dup, 0)), Remove(SelectDownstream(x), SelectUpstream(x))))}

% duplicate in upstream: {let dup = FindMatch(x, [""]) in Apply(Check(dup, [3]), Concat(Remove(SelectUpstream(x), SelectDup(dup, 3)), Remove(SelectDownstream(x), SelectUpstream(x))))}

% Freqpath: {let dup = FindMatch(x, ["base/logging.h"]) in Apply(Check(dup, [1]), Concat(Remove(SelectUpstream(x), SelectDownstreamPath(x, "base/logging.h")), Remove(SelectDownstream(x), SelectDownstreamPath(x, "base/logging.h"))))}

% freqpathupstream: {let dup = FindMatch(x, ["base/logging.h"]) in Apply(Check(dup, [1]), Concat(Remove(SelectDownstream(x), SelectDownstreamPath(x, "base/logging.h")), Remove(SelectUpstream(x), SelectDownstreamPath(x, "base/logging.h"))))}

% Dependencytest: {let dup = FindMatch(x, [""]) in Apply(Check(dup, [5, 7]), Concat(Remove(SelectDownstream(x), SelectDup(dup, 7)), Remove(SelectUpstream(x), SelectDownstream(x))))}

% downstream test: {let dup = FindMatch(x, [""]) in Apply(Check(dup, [5, 6]), Concat(Remove(SelectUpstream(x), SelectDup(dup, 6)), Remove(SelectDownstream(x), SelectUpstream(x))))}


%Sequence:
% 0: Duplicate in upstream and downstream
% 1: freqpattern
% 2: duplicate in downstream
% 3: duplicate in upstream
% 4: upstream specific
% 5: downstream specific
% 6: duplicate in downstream specific
% 7: dependency


%Macro:
%apply downstream: {let dup = FindMatch(x, [""]) in Apply(Check(dup, [5]), Remove(SelectDownstream(x), SelectUpstream(x)))}
% rename: {let dup = FindMatch(x, [""]) in Apply(Check(dup, []), Remove(SelectUpstream(x), SelectDownstream(x)))}


% Grammar:
% using Microsoft.ProgramSynthesis.Wrangling.Tree;
% using Microsoft.ProgramSynthesis.Transformation.Conflict.Learning;
% using Microsoft.ProgramSynthesis.Transformation.Conflict.Semantics;

% using semantics Microsoft.ProgramSynthesis.Transformation.Conflict.Semantics.Semantics;
% using learners Microsoft.ProgramSynthesis.Transformation.Conflict.Learning.Witnesses; 

% language Transformation.Conflict;

% @complete feature double Score = RankingScore;

% @input MergeConflict x;
% string path;
% string [] paths;
% int k;

% int[] enabledPredicate;

% @start IReadOnlyList<Node> proc:= rule;

% IReadOnlyList<Node> rule := @id['dupLet'] let dup: List<IReadOnlyList<Node>> = find in Apply(predicate, action);

% bool predicate := Check(dup, enabledPredicate);

% IReadOnlyList<Node> action  := Concat(action, action)
% 							|  Remove(t, t)
% 							|  t;

% IReadOnlyList<Node> t       := SelectUpstreamIdx(x, k)
%                             |  SelectUpstreamPath(x, path)
%                             |  SelectDownstreamIdx(x, k)
%                             |  SelectDownstreamPath(x, path)
%                             |  SelectDownstream(x)
%                             |  SelectUpstream(x)
% 							|  SelectDup(dup, k);

% List<IReadOnlyList<Node>> find	:= FindMatch(x, paths);

==> comments.tex <==
% Examples to demonstrate how did we design the DSL.
% Why program synthesis is needed instead of using classifier. (What ML would be returning for this problem)
% More transparent model
% Section V stronger.
% example -> DSL (Motivating examples)
% To-DO: FlashFill 
% Challenging example where simple concat wont work (in motivation section).
% Evaluate the power of the synthesis
% Random merge conflicts 

==> future.tex <==
\section{Future Impact and Implication of this work}
\label{sec:future}

==> motivation.tex <==
\section{Motivation for Program Synthesis}
\label{sec:motivation}


==> todo.tex <==
1. For scenarios, input program -done
2. Finish Bug fixing related work- done
3. Write the key features of the DSL (3 things)
4. Think a motivational example. -partially done
5. Write introduction

==> unseen-table.tex <==
\begin{table}
\centering
\caption{Results of Using Program Synthesis on \edge for 4 weeks dataset }
\label{tb:unseen}
\begin{tabular}{|l|c|c|}
\hline
\rowcolor{gray!35}
Pattern Name & Pattern Count & Successful \\ \hline
\hline
Concat       & 88            & 83 (94.3\%)        \\ \hline
\rowcolor{gray!25}
AFSC (Include)        & 5             & 4 (80.0\%)         \\ \hline
RD           & 12            & 11 (91.67\%)       \\ \hline
\rowcolor{gray!25}
FB           & 14            & 13 (92.8\%)        \\ \hline
DDC          & 6             & 5 (80.0\%)         \\ \hline
\rowcolor{gray!25}
Rename       & 15            & 14 (93.33\%)        \\ \hline
AFSC (Macro)  & 22            & 21 (95.4\%)        \\ \hline
\rowcolor{gray!25}
Total  & 162            & 151 (93.2\%)        \\ \hline
\end{tabular}
\end{table}
